FARE: Factor-Aware Retrieval with Error-Guided Fusion for Retail Forecasting

Retail sales forecasting underpins inventory planning, yet promotions and calendar events reshape short-term demand. Although each factor usually has historical occurrences, the complete factor combination of a target week often has few precedents. The challenge is therefore to retrieve informative partial matches and weight them by their reliability, which varies across series. We propose FARE(Factor-Aware Retrieval with Error-Guided Fusion), which ranks historical weeks separately for each known target-week factor and merges the selected weeks into a factor reference under a fixed budget. Guided by shrunk errors from completed development weeks and the current disagreement among candidates, a first gate mixes this factor reference with a shape reference from similar sales histories, and a second gate controls how strongly the mixture corrects a backbone forecast. Both gates remain fixed during testing. On Favorita, M5, Rossmann, and Rohlik, FARE reduces the weighted absolute percentage error (WAPE) of five backbones by 11.46%, 4.06%, 14.63%, and 10.16% on average. With Chronos-2 frozen, FARE also outperforms conventional and existing enhancement methods, including supervised residual correction and retrieval augmentation. Code is available at https://github.com/HousonGu/FARE .

==> author-info.tex <==
% Shared first-author footnote: *; corresponding-author footnote: dagger.
\makeatletter
\let\LLNCSOriginalFootnoteSymbol\@fnsymbol
\renewcommand{\@fnsymbol}[1]{%
  \ifnum#1=1\ensuremath{*}%
  \else\ifnum#1=2\ensuremath{\dagger}%
  \else\LLNCSOriginalFootnoteSymbol{#1}\fi\fi}
\makeatother

\makeatletter
\newcommand{\samefnsymbol}[1]{\textsuperscript{\@fnsymbol{#1}}}
\makeatother

\newcommand{\FirstAuthorEmail}{10245101426@stu.ecnu.edu.cn}
\newcommand{\SecondAuthorEmail}{10235101553@stu.ecnu.edu.cn}
\newcommand{\CorrespondingAuthorName}{}
\newcommand{\CorrespondingAuthorEmail}{}

% Keep LLNCS author counting, but print commas instead of "and".
\renewcommand{\andname}{\unskip,}
\renewcommand{\lastandname}{\unskip,}
\author{Chenghao Gu\inst{1}\thanks{Equal contribution.} \and
Zhuokang Shen\inst{1}\samefnsymbol{1} \and
Shenghao Wu\inst{1} \and
Tingxuan Zhu\inst{1}  \and
Weiyi Luo\inst{2} \and
Haifeng Tang\inst{2} \and%
\if\relax\expandafter\detokenize\expandafter{\CorrespondingAuthorName}\relax
\else
  \and \CorrespondingAuthorName\thanks{Corresponding author.}%
\fi
}
\authorrunning{C. Gu et al.}


\institute{East China Normal University, Shanghai, China
\and
China Merchants Bank Credit Card Center, Shanghai, China\\
\email{\FirstAuthorEmail, \SecondAuthorEmail}%
\if\relax\expandafter\detokenize\expandafter{\CorrespondingAuthorEmail}\relax
\else
  \\\email{\CorrespondingAuthorEmail}%
\fi
}

% Code link remains separate from the LLNCS author block.
\newcommand{\CodeRepositoryURL}{https://github.com/HousonGu/FARE}
\newcommand{\CodeRepositoryLink}{%
  \if\relax\expandafter\detokenize\expandafter{\CodeRepositoryURL}\relax
    \textit{Repository link pending}%
  \else
    \expandafter\url\expandafter{\CodeRepositoryURL}%
  \fi
}

